Near-Optimal Evasion of Convex-Inducing Classifiers

Classifiers are often used to detect miscreant activities. We study how an adversary can efficiently query a classifier to elicit information that allows the adversary to evade detection at near-minimal cost. We generalize results of Lowd and Meek (2005) to convex-inducing classifiers. We present algorithms that construct undetected instances of near-minimal cost using only polynomially many queries in the dimension of the space and without reverse engineering the decision boundary.

==> subfiles/discussion.tex <==
\section{DISCUSSION \& FUTURE WORK}
\label{sec:discuss}

The analysis of our algorithms shows that $\classSpace^\mathrm{convex}$ is
\kSearchable\ for weighted \LP[1] costs. When the positive class is
convex we demonstrated very efficient techniques that outperform the
previous reverse-engineering approaches for linear classifiers. When
the negative class is convex, we applied a randomized Ellipsoid method
to achieve efficient \kIMAC\ search. If the adversary is unaware
of which set is convex, they can trivially run both searches to
discover an \kIMAC\ with a combined polynomial query complexity.
%Our algorithms can also be efficiently extended to
%cope with a number of special circumstances (\eg\ if any feature
%weight $\ithCost{d}$ is infinite or if there is no initial lower bound
%\minCost\ on the \MAC) using preprocessing steps. These special cases
%will be explained in a longer version of the paper.

We have considered other \LP\ costs but it appears that
$\classSpace^{convex}$ is only \kSearchable\ for both positive and
negative convexity for any $\multGoal>0$ if $p=1$. For $0 < p < 1$,
the \MLS\ algorithms of Section~\ref{sec:pos-convex} achieve identical
results when the positive set is convex, but the non-convexity of
these \LP\ costs precludes the use of our randomized Ellipsoid method.
The Ellipsoid method does provide an efficient solution for convex
negative sets when $p>1$ (these costs are convex)---one only needs to
change the separating hyperplane of Eq.~\eqref{eq:gradient} with the
appropriate (sub)gradient of the desired \LP\ cost. However, for
convex positive sets, preliminary work suggests that solutions for
$p>1$ are generally not efficient.
%By using the \LP[1] ball as a bound on \LP[2] or \LP[\infty] balls, we
%found each to be \kSearchable[\sqrt{\dims}(1+\multGoal)] and
%\kSearchable[\dims(1+\multGoal)], respectively. 
%However, results based
%on packings suggust there are limits to query-based approaches for
%these costs.

\eat{
%Here we discuss the ramifications of our generalization of the near
%optimal evasion problem to \convexClass. 
As noted in Section~\ref{sec:opt-evasion}, we used a modified version
of near optimal evasion. We did not use the encoded sizes of
$\classifier$, $\dpt^+$, and $\dpt^-$ in defining \kSearchable\ as
these terms were unnecessary for our algorithms. Our approach also did
not use a third instance $\dpt^+ \in \xplus$ to simplify our \kIMAC\
search process.
%The rationale is that using $\xtarget$ in our search
%instead yields simpler search procedures. 
By using $\xtarget$ explicitly, our search is less \term{covert}
(easier to infer the attacker's intention form their queries) than
Lowd and Meek's approach, but by being less restrictive on the
adversary, we provide a worst-case analysis. Nonetheless,
incorporating covertness requirements remains a lucrative direction
for future work.
%(Covertness is not an explicit goal in \kIMAC\ search but it would be
%a requirement of many real-world attackers.)
%Since our goal was to analyze the best possible attack, covertness was
%ignored although it remains a lucrative direction for future work.
%is to study
%near optimal evasion with real-world covertness requirements.
}

% Secondly, using the encoded sizes of $\classifier$, $\dpt^+$, and
% $\dpt^-$ in defining \kSearchable\ is problematic. For our purposes,
% it is clear that the encoded size of both $\dpt^+$ and $\dpt^-$ is
% $\dims$ so it is unnecessary to include additional terms for their
% size. Further we allow for families of non-parametric classifiers for
% which the notion of \emph{encoding size} is ill-defined but is also
% unnecessary for the algorithms we present.
% % so we ignore that part of the definition. 
% %More importantly, in
% %extending beyond linear and parametric family of classifiers, it is
% %not straightforward to define the encoding size of our classifier
% %$\classifier$. One could use notions such as the \term{VC-dimension}
% %of $\classSpace$ or its \term{covering number} \ban{citations?} but it
% %is unclear why size of the classifier is important in quantifying the
% %complexity of \kIMAC\ search. Moreover, as we demonstrate in this
% %paper, there are non-parametric families of classifiers for which
% %\kIMAC\ search is polynomial in $\dims$ alone.  
% For this paper, we restrict our definition of \kSearchable\ to
% algorithms that require polynomially many queries in $\dims$ only.

% Finally, unlike Lowd and Meek's setting, in this paper we suppose that
% the adversary has only two initial instances, $\dpt^- \in \xminus$ and
% $\dpt^A$, eliminating the use of a third instance $\dpt^+ \in \xplus$.
% The rationale is that the adversary can determine the class of their
% desired instance $\dpt^A$ with only a single query to $\classifier$
% and it is the unique minimizer of $\adCost$. We restrict our setting
% to the case of $\dpt^A \in \xplus$; this yields simpler search
% procedures. However, as is apparent in the algorithms we demonstrate,
% using $\dpt^+ = \dpt^A$ makes the attacker less covert since it is
% significantly easier to infer the attacker's intentions based on their
% queries. (Covertness is not an explicit goal in \kIMAC\ search but it
% would be a requirement of many real-world attackers.) However, since
% our goal is not to design real attacks but rather analyze the best
% possible attack so as to understand our classifier's vulnerabilities,
% covertness can be ignored.

%%% TODO %%%
% \paragraph{Objections to ACRE Learnability}

% While several aspects of this problem were addressed by Lowd and Meek,
% some elements of their approach are undesirable. Namely, while ACRE Learnability is useful to broadly assess
% the vulnerability of a family of classifiers, there may be members of
% that family that are vulnerable to reverse engineering while others
% are not (\eg\ a family may not be $k$-ACRE Learnable for any
% $k$ but it may also subsume a family of $k$-ACRE Learnable
% classifiers such as linear classifiers). Thus, in practice, the
% classifier obtained from a particular training set may be vulnerable
% to efficient reverse engineering attacks even if it's from a family of
% classifiers that is not ACRE Learnable. Further, ACRE's minimization
% objective does not fully capture the motivation of realistic
% adversaries who merely want to find negative instances of low (but not
% necessarily minimal) cost. Thus, in our project, we explore algorithms
% that can find low-cost negative instances (while not necessarily
% minimal) for non-linear decision surfaces.


Exploring near optimal evasion is important for understanding
how an adversary may circumvent learners in security-sensitive
settings.
As described here, our algorithms may not always directly apply in practice
since 
%the feature space of a 
%learning algorithm is commonly secret.
%
%
% Discussion of real-world problems to near-optimal evasion; obtaining
% responses to queries, knowing the feature space, and reversing the
% feature mapping to submit real queries. Retraining
%Near-optimal evasion also 
various real-world obstacles persist. Queries may only be partially observable or noisy and
%classifiers may disallow querying; \eg\ spam filters
%rarely inform the sender when their message is classified as spam, but
%a spammer may obtain observability through dummy account. 
the feature set may only be partially known. Moreover,
an adversary may not be able to query all $\dpt \in
\xspace$. Queries must be objects (such as email) that
are mapped into $\xspace$. A real-world adversary must invert the
feature-mapping---a generally difficult task. These limitations necessitate
further research on the impact of partial observability and
approximate querying on \kIMAC\ search, and to design more secure filters.
%This
%context-dependent \term{query-observability} problem emphasizes that a
%real detector's security may be undermined if it's decisions are
%observable and that mechanisms for observability must be assessed.
%Similarly, 
%% There are also many interesting questions that remain about \kIMAC\
%% search. 
Broader open problems include: is \kIMAC\ search possible on
other classes of learners such as SVMs (linear in a large possibly
infinite feature space)? Is \kIMAC\ search feasible against an
online learner that adapts as it is queried?
%Second, is \kIMAC\ search possible when the adversary has restricted
%access to the full feature set? Third, could one reframe \kIMAC\
%search and the adversary's costs to operate in the space of real-world
%data by defining sets of legal operations to objects such as emails?
Can learners be made resilient to these threats and how does this
impact learning performance?
%how can learning benefit from \kIMAC\ search? How can
%vulnerabilities be eliminated once they have been identified and how
%does this affect the learner's performance?

%Mention Challenges to adversary in executing these attacks on
%real-learners: feature-space limitations \& reversing the map from
%real-world data to the instance space.

%%%% TODO %%%%
%\ban{Mention Challenges to good-guys in analyzing potential adversaries:
%lack of knowledge of the cost function, also reversing map for to
%real-world data, and finally how to retrain learners.}


==> subfiles/eval.tex <==
\section{Experiments}

Here we do several comparisons of the Linear Algorithm of Lowd \& Meek, our \emph{NEW} linear algorithm, our new algorithm for Convex Boundaries, and our general algorithm.

\subsection{Linear Boundary}

\subsection{Mandlebrot Boundary}

\subsection{SVMs}


==> subfiles/outline.tex <==
\newcommand{\TODO}{\emph{TODO:}}

\section{Outline}

\begin{enumerate}
\item \textbf{Introduction}
  \begin{enumerate}
  \item Explain why SecML is important
  \item Explain the concept of near-optimal evasion
  \item Explain the difference between reverse engineering (and active
    learning) and near-optimal evasion. Emphasize that near-optimal
    evasion is possible in cases where approximate reverse-engineering
    is not; in particular we demonstrate it for the convex set.s
  \end{enumerate}
\item \textbf{Problem Setup}
  \begin{enumerate}
  \item Terms to introduce
    \begin{enumerate}
    \item input space and label space. We only address real-valued
      finite dimensional input spaces.
    \item family of classifiers; \ie\ as a set of functions that map
      from input space to label space.
    \item family of cost functions
      \begin{itemize}
      \item Introduce weighted \LP\ distance based cost functions
      \item Emphasize that we are primarily interested in \LP[1] costs
      \item Emphasize that \LP[p] is convex for $p \ge 1$
      \end{itemize}
    \end{enumerate}
  \item Assumptions to present
    \begin{enumerate}
    \item The feature space is real-valued and finite dimensional
    \item The feature space is known to the adversary
    \item The family of classifiers is known to the adversary
    \item The classifier is a deterministic binary classifier
    \item The adversary can arbitrarily query any point in the feature
      space to determine it's label without reverse engineering the
      feature mapping.
    \item The adversary has at least 1 instance from both the positive
      and negative classes.
    \end{enumerate}
  \end{enumerate}
\item \textbf{ACRE (Near-optimal Evasion)}
  \begin{enumerate}
  \item Use the notion of minizing cost within the negative class with
    a minimal number of queries to motivate and formally define
    near-optimal evasion.
  \item Why does the complexity of the queries matter? Explain why
    this notion leads to a hardness but also what are the limitations
    of this analysis.
  \item Explain that restricting the family of classifiers is very
    important. Namely, show that, if we consider the family of all
    classifiers, finding a near-optimal instance is impossible.
  \item optimality (multiplicative \& additive)
    \begin{itemize}
    \item Explain why near-optimal evasion is formulated with
      multiplicative optimality; relative error reflects the fact that
      the adversary is willing to tolerate some factor of waste
      relative to the best cost they could possibly achieve.
    \item Emphasize that the two are similar; $A/B \le 1+\epsilon$
      is equivalent to $\log A - \log B \le \log(1+\epsilon)$.
    \item Emphasize that an algorithm that achieves
      $\delta$-additive optimality can be used to achieve
      $(1+\epsilon)$-multiplicative optimality by working
      converting to the log-space.
    \item Explain the ramification of multiplicative optimality that
      makes it very hard to find a near optimal instance when $C^\ast
      \approx 0$.
    \end{itemize}
  \item \TODO\ There is an important proposition we should prove;
    namely, that Query Optimization is harder than ordinary
    Optimization. That is, if an optimization problem is NP-Hard than
    it is NP-Hard to do via Query Optimization. This statement almost
    proves itself, but I don't have a formal proof.
  \end{enumerate}
\item \textbf{Extending to Convex (sic) Classifiers}
  \begin{enumerate}
    \item Case when positive class is convex
      \begin{itemize}
      \item We have a multi-line search algorithm that shows that
        search is efficient when the positive class is convex. Not
        only is this search polynomial, it is as efficient as
        reverse-engineering a linear classifier (\TODO\ we should
        emphasize this more by formally showing the complexity of Lowd
        \& Meek's algorithm). This is extraordinary in that the family
        of convex sets is much larger than the set of half-spaces
        (\TODO\ is there actually a countably argument here?).
        Certainly, it is intractible to sufficiently estimate the
        boundary of the convex set (\TODO\ we need a better
        explanation of this), but could it be done in a feasible
        neighborhood as was done by Lowd \& Meek; \TODO\ examine this
        possibility and compare it's complexity.
      \item We have a wide variety of different variants of multiline
        search including the shift from binary search to geometric
        search, Satish's $k$-steps of single line search and Steven's
        spiral search techniques. These improve on the original search
        and show theoretical improvements over the original multi-line
        search and the reverse-engineering techniques of Lowd \& Meek.
        In doing so, we further demonstrate that near-optimal evasion
        is easier reverse engineering.
      \item We finally have a lower-bound for both additive and
        multiplicative optimality. \TODO\ Some rewritting of these
        proofs should provide a clearer picture of what we're proving,
        but that should fit in with our overall explanation of
        additive vs. multiplicative optimality.
      \item \TODO\ As was suggest by NIPS Reviewer 1, our approach is
        limited to (weighted) \LP[1] costs; can we provide a more
        formal explanation of why it's amazing that it works for
        \LP[1] at all? In particular, I think it's possible to show
        NP-completeness for \LP[\infty] costs and perhaps even for
        \LP[2] costs. Maybe not for \LP[2]: I suggest applying a
        theorem of maximal bulging to attempt a polynomial algorithm,
        not for arbitrary $\epsilon$ but at least for some $epsilon$
        (perhaps dependent on the dimensionality of the space.
      \end{itemize}
    \item Case when positive class is convex
      \begin{itemize}
      \item We have a randomized algorithm that demonstrates a
        polynomial number of queries to find a near-optimal evasion
        point. This algorithm isn't particularly efficient but at
        least it's polynomial. \TODO\ We're in need of serious
        justification of why this case is harder.
      \item \TODO\ How many queries are required in practice.
      \item \TODO\ Is there a deterministic algorithm??? If not can we
        prove that no such algorithm is possible?
      \end{itemize}
    \item Case when it's unknown which class is convex
      \begin{itemize}
      \item The simple thing for the adversary to do is to run both
        algorithms above and use the best answer provided.
      \item \TODO\ Is there a more systematic way to deal with this
        case to combine the process of near-optimal optimization and
        determining which class is convex.
      \end{itemize}
  \end{enumerate}
\item \textbf{Extensions beyond Convexity}
  \begin{enumerate}
  \item Can we change the cost function from (weighted) \LP[1] costs?
    \begin{itemize}
    \item What about other \LP[p] distances? Special cases of \LP[2]
      and \LP[\infty] come to mind? What about general distances over
      the feature space?
    \item Are any of these cases NP-complete even with convex
      boundaries? Are there asymmetries between positive and negative
      convexity?
    \item What about cost functions that are not convex (and hence not
      distances). Possibly the most important is the minimum of
      several other cost functions.
    \end{itemize}
  \item Can we generalize near-optimal evasion to a broader family of
    classifiers? Are there other properties of a non-convex set that
    may be useful?
    \begin{itemize}
    \item Is there any hope for disconnected sets?
    \item What about connectedness?
    \item Is there an analog of Lipshitz for sets?
    \item What about SVMs? Is there some way to exploit the special
      structure of these decision functions?
    \end{itemize}
  \item In the general case, it may not be possible to ever guarantee
    near-optimal evasion.
    \begin{itemize}
    \item Consider the family of all possible decision functions\ldots
      it should be possible to show that this family can never be
      near-optimally evaded (even with some of the conditions we used
      for the convex set).
    \item In this case, all hope is not lost, there are still general
      purpose algorithms like our DiRect-based search. Clearly,
      though, such algorithms give up the guarantee of optimality and
      replace it with eventual optimality.
    \end{itemize}
  \end{enumerate}
\item \textbf{Experiments \& Practical Application}
  \begin{enumerate}
  \item Implementation of our algorithms.
    \begin{itemize}
    \item Detailed (and flexible) implementations of our convex
      positive algorithm is already available (thanks to Steven).
      \TODO\ We should make it a bit more flexible in various ways
      including allowing for non-homogonous feature costs.
    \end{itemize}
  \item Basic demonstration of practicality of our convex algorithms.
    \begin{itemize}
    \item Show that our convex positive algorithms really do use a
      small number of queries. Ideally, we'd like to be able to show
      that it outperforms the Lowd \& Meek algorithm on half-spaces.
    \item Show that our convex positive algorithm also works for truly
      convex sets such as the rectangles and ellipsoids we've been
      considering. \TODO\ We should think more about what sort of
      distribution to put on the ellipsoids.
    \item Show that our convex negative algorithm really is
      practically feasible to do near-optimal evasion with few
      queries.
    \end{itemize}
  \item Realistic (or pseudo-realistic) demonstration of near-optimal
    evasion.
    \begin{itemize}
    \item We need a realistic dataset such as spam with a meaningful
      set of features.
    \item We need to construct a realistic cost-function for these
      features.
    \item We need to have a good-approximation technique for reversing
      the mapping from feature space to input space.
    \item We need to be able to show (even if it's just a toy example)
      that our techniques could really produce a realistic and
      minimally changed spam.
    \end{itemize}
  \end{enumerate}
\item \textbf{Discussion}
  \begin{itemize}
  \item Reverse Engineering the boundary is overkill for the 
    near-optimal evasion problem.
  \item Our algorithms demonstrate that we can extend to boundaries
    of a convex set.
  \end{itemize}
\end{enumerate}

